Barriers in Seamless QoS for Mobile Applications

For seamless QoS, it is important that all the stakeholders, such as the hosts, applications, access networks, routers, and other middleboxes, follow a single protocol and they trust each other. In this article, we investigate the participation of these entities in providing QoS over wireless networks in light of DiffServ QoS architecture. We initiate the study by investigating WiFi and Cellular network traces, which further motivates us a thorough investigation of these stakeholders with empirical measurements. Our findings are the followings. (i) Modern mobile VoIP applications request QoS to the network. (ii) While the operating systems support basic APIs requesting QoS, application developers either are not aware of such requirements or they misuse the architecture for improved QoS. (iii) Wireless access networks rewrite the QoS requirements at the edge and enforce the rest of the routers or hops to provide best effort service. (iv) QoS requests are also nullified by the secure tunnels. (v) Although the access networks may nullify the QoS requests, the performance of the network still may differentiate traffic. We further emphasize that although the latest 5G network considers DiffServ QoS framework, it cannot deal with the challenges posed by the privacy related applications. Network neutrality is going to pose similar challenges.

==> backuprest/results.tex <==
\begin{table}[h!]
\begin{center}
{\footnotesize
 \begin{tabular}{| c | c | c | c | c | c | c |} 
 \hline
 \textbf{Network} & \textbf{CS0} & \textbf{AF31} & \textbf{AF33} & \textbf{AF41} & \textbf{AF43} & \textbf{EF} \\
 \hline
 MNO\#T  & 0\%  & 0\%  & NA  & 0\%  & 0\%  & 31.2\% \\
 \hline
 MNO\#1  & 0\% & 0\% & 0\%  & 0\%  & 0\%  & 0\%  \\ 
 \hline
 MNO\#2 & 0\%  & 0\%  & 46.0\%  & 0\%  & 43.0\%  & 27.7\%  \\
 \hline
  Wifi  & 0\% & 0\% & 0.008\%  & 0\%  & 0\%  & 0\%  \\ 
 \hline
\end{tabular}}
\caption{Maximum Loss Rates for local traces. \textcolor{red}{We need this for new amazon traces.} }
\label{table:remoteloss}
\end{center}
\end{table}

\begin{table}[h!]
\begin{center}
{\footnotesize
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
 Hupnet CS0, Hupnet AF33  & 0.0032709 & 0.03886079 & H\textsubscript{0} \\ 
 \hline
Hupnet CS0, Hupnet AF41 & 0.0043363 & 0.03897706  & H\textsubscript{0} \\  
 \hline
Hupnet CS0, Hupnet AF43 & 0.0033131 & 0.03892957  & H\textsubscript{0} \\
  \hline
Hupnet CS0, Hupnet CS6 & 0.9996 & 0.03884237  & H\textsubscript{1} \\
  \hline
Hupnet CS0, Hupnet EF & 1 & 0.03892645  & H\textsubscript{1} \\
 \hline
\end{tabular}}
\caption{Hupnet Network KS Test Result}
\label{table:hupnetks}
\end{center}
\end{table}




\begin{figure*}[!h]
\centering
\includegraphics[width=0.325\linewidth]{images/hupnet_local.pdf}
\includegraphics[width=0.325\linewidth]{images/sonera_local.pdf}
\includegraphics[width=0.325\linewidth]{images/sauna_local.pdf}
\caption{Ecdf Graph for Hupnet }
\label{fig:hupnetecdf}
\end{figure*}



\begin{table}[h!]
\begin{center}
{\footnotesize
 \begin{tabular}{| c | c | c | c | c | c | c |} 
 \hline
 \textbf{Network} & \textbf{CS0} & \textbf{AF31} & \textbf{AF33} & \textbf{AF41} & \textbf{AF43} & \textbf{EF} \\
 \hline
 MNO\#T  & 0\%  & 0\%  & NA  & 0\%  & 0\%  & 31.2\% \\
 \hline
 MNO\#1  & 0\% & 0\% & 0\%  & 0\%  & 0\%  & 0\%  \\ 
 \hline
 MNO\#2 & 0\%  & 0\%  & 46.0\%  & 0\%  & 43.0\%  & 27.7\%  \\
 \hline
  Wifi  & 0\% & 0\% & 0.008\%  & 0\%  & 0\%  & 0\%  \\ 
 \hline
\end{tabular}}
\caption{Maximum Loss Rates for local traces. \textcolor{red}{We need this for new local traces.} }
\label{table:localloss}
\end{center}
\end{table}

\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
  Sauna CS0, Sauna AF31  & 0.00079968 & 0.03846276 & H\textsubscript{0} \\ 
 \hline
 Sauna CS0, Sauna AF33  & 0.0019992 & 0.03846661 & H\textsubscript{0} \\ 
 \hline
Sauna CS0, Sauna AF41 & 0.0019992 & 0.03845892  & H\textsubscript{0} \\  
 \hline
Sauna CS0, Sauna AF43 & 0.002399 & 0.03846276  & H\textsubscript{0} \\
  \hline
Sauna CS0, Sauna CS6 & 0.9972 & 0.03845892  & H\textsubscript{1} \\
  \hline
Sauna CS0, Sauna EF & 0.5008 & 0.03329975  & H\textsubscript{1} \\
 \hline
\end{tabular}
\caption{Saunalahti Network KS Test Result}
\label{table:saunaks}
\end{center}


\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
  Sonera CS0, Sonera AF31  & 0.0019986 & 0.03847432 & H\textsubscript{0} \\ 
 \hline
 Sonera CS0, Sonera AF33  & 0.0023963 & 0.03845507 & H\textsubscript{0} \\ 
 \hline
Sonera CS0, Sonera AF41 & 0.0027984 & 0.03846276  & H\textsubscript{0} \\  
 \hline
Sonera CS0, Sonera AF43 & 0.0031942 & 0.03845123  & H\textsubscript{0} \\
  \hline
Sonera CS0, Sonera CS6 & 0.9976 & 0.03845892  & H\textsubscript{1} \\
  \hline
Sonera CS0, Sonera EF & 1 & 0.03845892  & H\textsubscript{1} \\
 \hline
\end{tabular}
\caption{Sonera Network KS Test Result}
\label{table:soneraks}
\end{center}
\end{table}




\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
Hupnet CS0-1, Hupnet AF31  & 0.0033198 &  0.03852457 & H\textsubscript{0} \\ 
\hline
Hupnet CS0-1 and Hupnet AF33  & 1 &  0.03886492 & H\textsubscript{1} \\ 
\hline
Hupnet CS0-1 and Hupnet AF41  & 1 &  0.03897747 & H\textsubscript{1} \\ 
\hline
Hupnet CS0-1 and Hupnet AF43  & 1 &  0.03891467 & H\textsubscript{1} \\ 
\hline
Hupnet CS0-1 and Hupnet EF  & 1 &  0.038923 & H\textsubscript{1} \\ 
\hline
Hupnet CS0-1 and Hupnet CS6  & 1 &  0.03881969 & H\textsubscript{1} \\ 
\hline
Hupnet CS0-2 and Hupnet AF31  & 1 &  0.03852457 & H\textsubscript{1} \\ 
\hline
Hupnet CS0-2 and Hupnet AF33  & 0.0035851 &  0.03886492 & H\textsubscript{0} \\ 
\hline
Hupnet CS0-2 and Hupnet AF41  & 1 &  0.03897747 & H\textsubscript{1} \\ 
\hline
Hupnet CS0-2 and Hupnet AF43  & 1 &  0.03891467 & H\textsubscript{1} \\ 
\hline
Hupnet CS0-2 and Hupnet EF  & 1 &  0.038923 & H\textsubscript{1} \\ 
\hline
 Hupnet CS0-2 and Hupnet CS6  & 1 & 0.03881969 & H\textsubscript{1} \\ 
\hline
Hupnet CS0-3 and Hupnet AF31 & 1 & 0.03852842  & H\textsubscript{1} \\  
\hline
Hupnet CS0-3 and Hupnet AF33 & 1 & 0.03886873  & H\textsubscript{1} \\  
\hline
Hupnet CS0-3 and Hupnet AF41 & 0.0045823 & 0.03898127  & H\textsubscript{0} \\  
\hline
Hupnet CS0-3 and Hupnet AF43 & 1 & 0.03891847  & H\textsubscript{1} \\  
\hline
Hupnet CS0-3 and Hupnet EF & 1 & 0.03892681  & H\textsubscript{1} \\  
\hline
Hupnet CS0-3 and Hupnet CS6 & 1 & 0.03882351  & H\textsubscript{1} \\  
\hline
Hupnet CS0-4 and Hupnet AF31 & 1 & 0.03852842  & H\textsubscript{1} \\ 
\hline
Hupnet CS0-4 and Hupnet AF33 & 1 & 0.038884  & H\textsubscript{1} \\  
\hline
Hupnet CS0-4 and Hupnet AF41 & 1 & 0.0389965  & H\textsubscript{1} \\  
\hline
Hupnet CS0-4 and Hupnet AF43 & 0.0035315 & 0.03893373  & H\textsubscript{0} \\  
\hline
Hupnet CS0-4 and Hupnet EF & 1 & 0.03894206  & H\textsubscript{1} \\  
\hline
Hupnet CS0-4 and Hupnet CS6 & 1 & 0.0388388  & H\textsubscript{1} \\  
\hline
Hupnet CS0-5 and Hupnet AF31 & 1 & 0.03855154  & H\textsubscript{1} \\ 
\hline
Hupnet CS0-5 and Hupnet AF33 & 1 & 0.03889165  & H\textsubscript{1} \\  
\hline
Hupnet CS0-5 and Hupnet AF41 & 1 & 0.03900413  & H\textsubscript{1} \\  
\hline
Hupnet CS0-5 and Hupnet AF43 & 1 & 0.03894137  & H\textsubscript{1} \\  
\hline
Hupnet CS0-5 and Hupnet EF & 0.0029125 & 0.0389497  & H\textsubscript{0} \\  
\hline
Hupnet CS0-5 and Hupnet CS6 & 1 & 0.03884646  & H\textsubscript{1} \\  
\hline
Hupnet CS0-6 and Hupnet AF31 & 1 & 0.03853226  & H\textsubscript{1} \\ 
\hline
Hupnet CS0-6 and Hupnet AF33 & 1 & 0.03887254  & H\textsubscript{1} \\  
\hline
Hupnet CS0-6 and Hupnet AF41 & 1 & 0.03898507  & H\textsubscript{1} \\  
\hline
Hupnet CS0-6 and Hupnet AF43 & 1 & 0.03892228  & H\textsubscript{1} \\  
\hline
Hupnet CS0-6 and Hupnet EF & 1 & 0.03893061  & H\textsubscript{1} \\  
\hline
Hupnet CS0-6 and Hupnet CS6 & 0.0050251 & 0.03882733  & H\textsubscript{0} \\  
\hline
\end{tabular}
\caption{Hupnet Local Network KS Test Result}
\label{table:huks}
\end{center}
\end{table}



\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
Sauna CS0-1 and Sauna AF31  & 0.00039984 &  0.03845892 & H\textsubscript{0} \\ 
\hline
Sauna CS0-1 and Sauna AF33  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sauna CS0-1 and Sauna AF41  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sauna CS0-1 and Sauna AF43  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sauna CS0-1 and Sauna EF  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sauna CS0-1 and Sauna CS6  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sauna CS0-2 and Sauna AF31  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sauna CS0-2 and Sauna AF33  & 0.00039984 &  0.03845892 & H\textsubscript{0} \\ 
\hline
Sauna CS0-2 and Sauna AF41  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sauna CS0-2 and Sauna AF43  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sauna CS0-2 and Sauna EF  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
 Sauna CS0-2 and Sauna CS6  & 1 & 0.03845892 & H\textsubscript{1} \\ 
\hline
Sauna CS0-3 and Sauna AF31 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-3 and Sauna AF33 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-3 and Sauna AF41 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\  
\hline
Sauna CS0-3 and Sauna AF43 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-3 and Sauna EF & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-3 and Sauna CS6 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-4 and Sauna AF31 & 1 & 0.03845892  & H\textsubscript{1} \\ 
\hline
Sauna CS0-4 and Sauna AF33 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-4 and Sauna AF41 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-4 and Sauna AF43 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\  
\hline
Sauna CS0-4 and Sauna EF & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-4 and Sauna CS6 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-5 and Sauna AF31 & 1 & 0.03845892  & H\textsubscript{1} \\ 
\hline
Sauna CS0-5 and Sauna AF33 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-5 and Sauna AF41 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-5 and Sauna AF43 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-5 and Sauna EF & 0.00039984 & 0.03845892  & H\textsubscript{0} \\  
\hline
Sauna CS0-5 and Sauna CS6 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-6 and Sauna AF31 & 1 & 0.03845892  & H\textsubscript{1} \\ 
\hline
Sauna CS0-6 and Sauna AF33 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-6 and Sauna AF41 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-6 and Sauna AF43 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-6 and Sauna EF & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sauna CS0-6 and Sauna CS6 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\  
\hline
\end{tabular}
\caption{Sauna Local Network KS Test Result}
\label{table:saunaks}
\end{center}
\end{table}

\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
Sonera CS0-1 and Sonera AF31  & 0.00079968 &  0.03845892 & H\textsubscript{0} \\ 
\hline
Sonera CS0-1 and Sonera AF33  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-1 and Sonera AF41  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-1 and Sonera AF43  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-1 and Sonera EF  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-1 and Sonera CS6  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-2 and Sonera AF31  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-2 and Sonera AF33  & 0.00079968 &  0.03845892 & H\textsubscript{0} \\ 
\hline
Sonera CS0-2 and Sonera AF41  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-2 and Sonera AF43  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-2 and Sonera EF  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
 Sonera CS0-2 and Sonera CS6  & 1 & 0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-3 and Sonera AF31 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-3 and Sonera AF33 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-3 and Sonera AF41 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\  
\hline
Sonera CS0-3 and Sonera AF43 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-3 and Sonera EF & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-3 and Sonera CS6 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-4 and Sonera AF31 & 1 & 0.03845892  & H\textsubscript{1} \\ 
\hline
Sonera CS0-4 and Sonera AF33 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-4 and Sonera AF41 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-4 and Sonera AF43 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\  
\hline
Sonera CS0-4 and Sonera EF & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-4 and Sonera CS6 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-5 and Sonera AF31 & 1 & 0.03845892  & H\textsubscript{1} \\ 
\hline
Sonera CS0-5 and Sonera AF33 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-5 and Sonera AF41 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-5 and Sonera AF43 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-5 and Sonera EF & 0.00079968 & 0.03845892  & H\textsubscript{0} \\  
\hline
Sonera CS0-5 and Sonera CS6 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-6 and Sonera AF31 & 1 & 0.03845892  & H\textsubscript{1} \\ 
\hline
Sonera CS0-6 and Sonera AF33 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-6 and Sonera AF41 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-6 and Sonera AF43 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-6 and Sonera EF & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-6 and Sonera CS6 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\  
\hline
\end{tabular}
\caption{Sonera Local Network KS Test Result}
\label{table:Soneraks}
\end{center}
\end{table}


\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
Wifi CS0-1 and Wifi AF31  & 0.0012479 &  0.03847432 & H\textsubscript{0} \\ 
\hline
Wifi CS0-1 and Wifi AF33  & 1 &  0.03846276 & H\textsubscript{1} \\ 
\hline
Wifi CS0-1 and Wifi AF41  & 1 &  0.03847432 & H\textsubscript{1} \\ 
\hline
Wifi CS0-1 and Wifi AF43  & 1 &  0.03847817 & H\textsubscript{1} \\ 
\hline
Wifi CS0-1 and Wifi EF  & 1 &  0.03850137 & H\textsubscript{1} \\ 
\hline
Wifi CS0-1 and Wifi CS6  & 1 &  0.03846276 & H\textsubscript{1} \\ 
\hline
Wifi CS0-2 and Wifi AF31  & 1 &  0.03847432 & H\textsubscript{1} \\ 
\hline
Wifi CS0-2 and Wifi AF33  & 0.00076433 &  0.03846276 & H\textsubscript{0} \\ 
\hline
Wifi CS0-2 and Wifi AF41  & 1 &  0.03847432 & H\textsubscript{1} \\ 
\hline
Wifi CS0-2 and Wifi AF43  & 1 &  0.03847817 & H\textsubscript{1} \\ 
\hline
Wifi CS0-2 and Wifi EF  & 1 &  0.03850137 & H\textsubscript{1} \\ 
\hline
 Wifi CS0-2 and Wifi CS6  & 1 & 0.03846276 & H\textsubscript{1} \\ 
\hline
Wifi CS0-3 and Wifi AF31 & 1 & 0.03847432  & H\textsubscript{1} \\  
\hline
Wifi CS0-3 and Wifi AF33 & 1 & 0.03846276  & H\textsubscript{1} \\  
\hline
Wifi CS0-3 and Wifi AF41 & 0.0010133 & 0.03847432  & H\textsubscript{0} \\  
\hline
Wifi CS0-3 and Wifi AF43 & 1 & 0.03847817  & H\textsubscript{1} \\  
\hline
Wifi CS0-3 and Wifi EF & 1 & 0.03850137  & H\textsubscript{1} \\  
\hline
Wifi CS0-3 and Wifi CS6 & 1 & 0.03846276  & H\textsubscript{1} \\  
\hline
Wifi CS0-4 and Wifi AF31 & 1 & 0.03847432  & H\textsubscript{1} \\ 
\hline
Wifi CS0-4 and Wifi AF33 & 1 & 0.03846276  & H\textsubscript{1} \\  
\hline
Wifi CS0-4 and Wifi AF41 & 1 & 0.03847432  & H\textsubscript{1} \\  
\hline
Wifi CS0-4 and Wifi AF43 & 0.0012232 & 0.03847817  & H\textsubscript{0} \\  
\hline
Wifi CS0-4 and Wifi EF & 1 & 0.03850137  & H\textsubscript{1} \\  
\hline
Wifi CS0-4 and Wifi CS6 & 1 & 0.03846276  & H\textsubscript{1} \\  
\hline
Wifi CS0-5 and Wifi AF31 & 1 & 0.03847432  & H\textsubscript{1} \\ 
\hline
Wifi CS0-5 and Wifi AF33 & 1 & 0.03846276  & H\textsubscript{1} \\  
\hline
Wifi CS0-5 and Wifi AF41 & 1 & 0.03847432  & H\textsubscript{1} \\  
\hline
Wifi CS0-5 and Wifi AF43 & 1 & 0.03850137  & H\textsubscript{1} \\  
\hline
Wifi CS0-5 and Wifi EF & 0.0022634 & 0.03846276  & H\textsubscript{0} \\  
\hline
Wifi CS0-5 and Wifi CS6 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Wifi CS0-6 and Wifi AF31 & 1 & 0.03847432  & H\textsubscript{1} \\ 
\hline
Wifi CS0-6 and Wifi AF33 & 1 & 0.03846276  & H\textsubscript{1} \\  
\hline
Wifi CS0-6 and Wifi AF41 & 1 & 0.03847432  & H\textsubscript{1} \\  
\hline
Wifi CS0-6 and Wifi AF43 & 1 & 0.03847817  & H\textsubscript{1} \\  
\hline
Wifi CS0-6 and Wifi EF & 1 & 0.03850137  & H\textsubscript{1} \\  
\hline
Wifi CS0-6 and Wifi CS6 & 0.0019517 & 0.03846276  & H\textsubscript{0} \\  
\hline
\end{tabular}
\caption{Wifi Remote Network KS Test Result}
\label{table:Wifiks}
\end{center}
\end{table}


\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
Elisa CS0-1 and Elisa AF31  & 0.016952 &  0.03884134 & H\textsubscript{0} \\ 
\hline
Elisa CS0-1 and Elisa AF33  & 1 &  0.03905186 & H\textsubscript{1} \\ 
\hline
Elisa CS0-1 and Elisa AF41  & 1 &  0.03863468 & H\textsubscript{1} \\ 
\hline
Elisa CS0-1 and Elisa AF43  & 1 &  0.0388136 & H\textsubscript{1} \\ 
\hline
Elisa CS0-1 and Elisa EF  & 1 &  0.0388136 & H\textsubscript{1} \\ 
\hline
Elisa CS0-1 and Elisa CS6  & 1 &  0.03906425 & H\textsubscript{1} \\ 
\hline
Elisa CS0-2 and Elisa AF31  & 1 &  0.03908336 & H\textsubscript{1} \\ 
\hline
Elisa CS0-2 and Elisa AF33  & 0.0041736 &  0.03929258 & H\textsubscript{0} \\ 
\hline
Elisa CS0-2 and Elisa AF41  & 1 &  0.03887798 & H\textsubscript{1} \\ 
\hline
Elisa CS0-2 and Elisa AF43  & 1 &  0.03905579 & H\textsubscript{1} \\ 
\hline
Elisa CS0-2 and Elisa EF  & 1 &  0.03905579 & H\textsubscript{1} \\ 
\hline
 Elisa CS0-2 and Elisa CS6  & 1 & 0.03930489 & H\textsubscript{1} \\ 
\hline
Elisa CS0-3 and Elisa AF31 & 1 & 0.03866652  & H\textsubscript{1} \\  
\hline
Elisa CS0-3 and Elisa AF33 & 1 & 0.03887798  & H\textsubscript{1} \\  
\hline
Elisa CS0-3 and Elisa AF41 & 0.00079968 & 0.03845892  & H\textsubscript{0} \\  
\hline
Elisa CS0-3 and Elisa AF43 & 1 & 0.03863865  & H\textsubscript{1} \\  
\hline
Elisa CS0-3 and Elisa EF & 1 & 0.03863865  & H\textsubscript{1} \\  
\hline
Elisa CS0-3 and Elisa CS6 & 1 & 0.03889043  & H\textsubscript{1} \\  
\hline
Elisa CS0-4 and Elisa AF31 & 1 & 0.0388532  & H\textsubscript{1} \\ 
\hline
Elisa CS0-4 and Elisa AF33 & 1 & 0.03906365  & H\textsubscript{1} \\  
\hline
Elisa CS0-4 and Elisa AF41 & 1 & 0.0386466  & H\textsubscript{1} \\  
\hline
Elisa CS0-4 and Elisa AF43 & 0.0047181 & 0.03882546  & H\textsubscript{0} \\  
\hline
Elisa CS0-4 and Elisa EF & 1 & 0.03882546  & H\textsubscript{1} \\  
\hline
Elisa CS0-4 and Elisa CS6 & 1 & 0.03907603  & H\textsubscript{1} \\  
\hline
Elisa CS0-5 and Elisa AF31 & 1 & 0.03884134  & H\textsubscript{1} \\ 
\hline
Elisa CS0-5 and Elisa AF33 & 1 & 0.03905186  & H\textsubscript{1} \\  
\hline
Elisa CS0-5 and Elisa AF41 & 1 & 0.03863468  & H\textsubscript{1} \\  
\hline
Elisa CS0-5 and Elisa AF43 & 1 & 0.0388136  & H\textsubscript{1} \\  
\hline
Elisa CS0-5 and Elisa EF & 0.0042136 & 0.0388136  & H\textsubscript{0} \\  
\hline
Elisa CS0-5 and Elisa CS6 & 1 & 0.03906425  & H\textsubscript{1} \\  
\hline
Elisa CS0-6 and Elisa AF31 & 1 & 0.039104  & H\textsubscript{1} \\ 
\hline
Elisa CS0-6 and Elisa AF33 & 1 & 0.03931311  & H\textsubscript{1} \\  
\hline
Elisa CS0-6 and Elisa AF41 & 1 & 0.03889874  & H\textsubscript{1} \\  
\hline
Elisa CS0-6 and Elisa AF43 & 1 & 0.03907645  & H\textsubscript{1} \\  
\hline
Elisa CS0-6 and Elisa EF & 1 & 0.03907645  & H\textsubscript{1} \\  
\hline
Elisa CS0-6 and Elisa CS6 & 0.0041645 & 0.03932542  & H\textsubscript{0} \\  
\hline
\end{tabular}
\caption{Elisa Remote Network KS Test Result}
\label{table:Elisaks}
\end{center}
\end{table}


\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
Sonera CS0-1 and Sonera AF31  & 0.00039984 &  0.03845892 & H\textsubscript{0} \\ 
\hline
Sonera CS0-1 and Sonera AF33  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-1 and Sonera AF41  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-1 and Sonera AF43  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-1 and Sonera EF  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-1 and Sonera CS6  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-2 and Sonera AF31  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-2 and Sonera AF33  & 0.00079968 &  0.03845892 & H\textsubscript{0} \\ 
\hline
Sonera CS0-2 and Sonera AF41  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-2 and Sonera AF43  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-2 and Sonera EF  & 1 &  0.03845892 & H\textsubscript{1} \\ 
\hline
 Sonera CS0-2 and Sonera CS6  & 1 & 0.03845892 & H\textsubscript{1} \\ 
\hline
Sonera CS0-3 and Sonera AF31 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-3 and Sonera AF33 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-3 and Sonera AF41 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\  
\hline
Sonera CS0-3 and Sonera AF43 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-3 and Sonera EF & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-3 and Sonera CS6 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-4 and Sonera AF31 & 1 & 0.03845892  & H\textsubscript{1} \\ 
\hline
Sonera CS0-4 and Sonera AF33 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-4 and Sonera AF41 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-4 and Sonera AF43 & 0.002399 & 0.03845892  & H\textsubscript{0} \\  
\hline
Sonera CS0-4 and Sonera EF & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-4 and Sonera CS6 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-5 and Sonera AF31 & 1 & 0.03845892  & H\textsubscript{1} \\ 
\hline
Sonera CS0-5 and Sonera AF33 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-5 and Sonera AF41 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-5 and Sonera AF43 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-5 and Sonera EF & 0.00039984 & 0.03845892  & H\textsubscript{0} \\  
\hline
Sonera CS0-5 and Sonera CS6 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-6 and Sonera AF31 & 1 & 0.03845892  & H\textsubscript{1} \\ 
\hline
Sonera CS0-6 and Sonera AF33 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-6 and Sonera AF41 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-6 and Sonera AF43 & 1 & 0.03845892  & H\textsubscript{1} \\  
\hline
Sonera CS0-6 and Sonera EF & 1 & 0.00039984  & H\textsubscript{1} \\  
\hline
Sonera CS0-6 and Sonera CS6 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\  
\hline
\end{tabular}
\caption{Sonera Remote Network KS Test Result}
\label{table:Soneraks}
\end{center}
\end{table}

\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
  Wifi CS0, Wifi AF31  & 0.0012479 & 0.03847432 & H\textsubscript{0} \\ 
 \hline
 Wifi CS0, Wifi AF33  & 0.00076433 & 0.03846276 & H\textsubscript{0} \\ 
 \hline
Wifi CS0, Wifi AF41 & 0.0010133 & 0.03847432  & H\textsubscript{0} \\  
 \hline
Wifi CS0, Wifi AF43 & 0.0012232 & 0.03847817  & H\textsubscript{0} \\
  \hline
Wifi CS0, Wifi EF & 0.0022634 & 0.03850137  & H\textsubscript{0} \\
 \hline
 Wifi CS0, Wifi CS6 & 0.0019517 & 0.03846276  & H\textsubscript{0} \\
  \hline
\end{tabular}
\caption{Wifi Remote Network KS Test Result}
\label{table:wifiks}
\end{center}
\end{table}

\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
  Elisa CS0, Elisa AF31  & 0.016952 & 0.03884134 & H\textsubscript{0} \\ 
 \hline
 Elisa CS0, Elisa AF33  & 0.0041736 & 0.03929258 & H\textsubscript{0} \\ 
 \hline
Elisa CS0, Elisa AF41 & 0.00079968 & 0.03845892  & H\textsubscript{0} \\  
 \hline
Elisa CS0, Elisa AF43 & 0.0047181 & 0.03882546  & H\textsubscript{0} \\
  \hline
Elisa CS0, Elisa EF & 0.0042136 & 0.0388136  & H\textsubscript{0} \\
 \hline
 Elisa CS0, Elisa CS6 & 0.0041645 & 0.03932542  & H\textsubscript{0} \\
  \hline
\end{tabular}
\caption{Elisa Remote Network KS Test Result}
\label{table:elisaks}
\end{center}
\end{table}

\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
  Sonera CS0, Sonera AF31  & 0.00039984 & 0.03845892 & H\textsubscript{0} \\ 
 \hline
 Sonera CS0, Sonera AF33  & 0.00079968 & 0.03845892 & H\textsubscript{0} \\ 
 \hline
Sonera CS0, Sonera AF41 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\  
 \hline
Sonera CS0, Sonera AF43 & 0.002399 & 0.03845892  & H\textsubscript{0} \\
  \hline
Sonera CS0, Sonera EF & 0.00039984 & 0.03845892  & H\textsubscript{0} \\
 \hline
Sonera CS0, Sonera CS6 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\
  \hline
\end{tabular}
\caption{Sonera Remote Network KS Test Result}
\label{table:elisaks}
\end{center}
\end{table}

\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
Hupnet CS0, Hupnet AF31  & 0.0033198 &  0.03852457 & H\textsubscript{0} \\ 
\hline
 Hupnet CS0, Hupnet AF33  & 0.0035851 & 0.03886492 & H\textsubscript{0} \\ 
\hline
Hupnet CS0, Hupnet AF41 & 0.0045823 & 0.03898127  & H\textsubscript{0} \\  
\hline
Hupnet CS0, Hupnet AF43 & 0.0035315 & 0.03893373  & H\textsubscript{0} \\
 \hline
Hupnet CS0, Hupnet EF & 0.0029125 & 0.0389497  & H\textsubscript{0} \\
\hline
Hupnet CS0, Hupnet CS6 & 0.0050251 & 0.03882733  & H\textsubscript{0} \\
 \hline
\end{tabular}
\caption{Hupnet Network KS Test Result}
\label{table:hupnetks}
\end{center}
\end{table}

\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
  Sauna CS0, Sauna AF31  & 0.00039984 & 0.03845892 & H\textsubscript{0} \\ 
 \hline
 Sauna CS0, Sauna AF33  & 0.00039984 & 0.03845892 & H\textsubscript{0} \\ 
 \hline
Sauna CS0, Sauna AF41 & 0.00039984 & 0.03845892 & H\textsubscript{0} \\ 
 \hline
Sauna CS0, Sauna AF43 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\
  \hline
Sauna CS0, Sauna EF & 0.00039984 & 0.03845892   & H\textsubscript{0} \\
 \hline
 Sauna CS0, Sauna CS6 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\
  \hline
\end{tabular}
\caption{Saunalahti Network KS Test Result}
\label{table:saunaks}
\end{center}
\end{table}

\begin{table}[h!]
\begin{center}
 \begin{tabular}{| c | c | c | c | c |} 
 \hline
 \textbf{Data Sets} & \textbf{D\textsubscript{x,y}} & \textbf{C($\alpha$}) & \textbf{Accepted} \\ 
 \hline
  Sonera CS0, Sonera AF31  & 0.00079968 & 0.03845892 & H\textsubscript{0} \\ 
 \hline
 Sonera CS0, Sonera AF33  & 0.00079968 & 0.03845892 & H\textsubscript{0} \\ 
 \hline
Sonera CS0, Sonera AF41 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\  
 \hline
Sonera CS0, Sonera AF43 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\
  \hline
Sonera CS0, Sonera EF & 0.00079968 & 0.03845892  & H\textsubscript{0} \\
 \hline
 Sonera CS0, Sonera CS6 & 0.00039984 & 0.03845892  & H\textsubscript{0} \\
  \hline
\end{tabular}
\caption{Sonera Network KS Test Result}
\label{table:soneraks}
\end{center}
\end{table}






==> imagetexes/netintpacket.tex <==

    \begin{tikzpicture}[baseline] 
        \begin{groupplot}[group style={group size=4 by 1, horizontal sep=5em, vertical sep=5em}]


           \nextgroupplot[
        legend pos=north west,
        legend cell align=left,
%		title=the impact of Memory on Executor Size,
%		xlabel=Executor size,
		ylabel=Running Time(100Sec),
		label style={font=\Huge},
		title style={font=\Huge},
		legend style={font=\Large},
		ymax=6,
		ytick={0,0.1,...,1},
		xtick={0,1,...,10},
		xticklabels={size1,size2,size3,size4,size5},
		]
		
	
	
  \addplot [smooth, blue] {normcdf(x,0,4)};
  \addplot [smooth, black] {normcdf(x,0,2)};

  \legend{Wordcount,Sort,Terasort}

            \nextgroupplot[
        legend pos=north east,
        legend cell align=left,
%		title=the impact of Memory on Executor Size,
		xlabel=Executor size,
		ylabel=GC time/Total time (\%),
		label style={font=\Huge},
		title style={font=\Huge},
		legend style={font=\Large},
		ymax=40,
		ytick={0,10,...,40},
		xtick={1,2,...,6},
		xticklabels={size1,size2,size3,size4,size5,size6},
		]
		
		\addplot[color=blue,mark=o,mark size=4pt,ultra thick] coordinates {
(1,1.0443745360000203)
(2,1.2312978969185548)
(3,1.6321503318209594)
(4,1.6223729700821123)
(5,1.5582041400952296)
(6,0.9600154370109788)
	};
	
		\addplot[color=purple,mark=x, mark size=4pt,ultra thick] coordinates {

(1,7.25805417718133)
(2,5.1081969273646255)
(3,4.917338539093479)
(4,2.330211280160177)
(5,1.3883373674768877)
(6,0.5960967436140351)

	};
	
	\addplot[color=black,mark=triangle,mark size=4pt,ultra thick] coordinates {
    
(1,15.689213470100041)
(2,10.853722407648753)
(3,9.777287357940002)
(4,5.663117872329123)
(5,3.243273011304715)
(6,1.4751343408080855)
	};		

\legend{Wordcount,Sort,Terasort}

      \nextgroupplot[
        legend pos=north east,
        legend cell align=left,
%		title=the impact of Memory on Executor Size,
		xlabel=Executor size,
		ylabel=GC time/Total time (\%),
		label style={font=\Huge},
		title style={font=\Huge},
		legend style={font=\Large},
		ymax=40,
		ytick={0,10,...,40},
		xtick={1,2,...,6},
		xticklabels={size1,size2,size3,size4,size5,size6},
		]
		
	
%4	
		\addplot[color=blue,mark=o,mark size=4pt,ultra thick] coordinates {
(1,26.25207854059642)
(2,26.36121853795766)
(3,17.708051594671286)
(4,13.68865105536088)
(5,11.328440987284013)
(6,12.603772400405532)


	};		
%5
		\addplot[color=purple,mark=x, mark size=4pt,ultra thick] coordinates {
(1,4.648002362391365)
(2,4.344727424580203)
(3,3.588342192249632)
(4,3.2608538140611936)
(5,2.5259182901903334)
(6,1.8564070460456334)

	};	
	%6
	\addplot[color=black,mark=triangle,mark size=4pt,ultra thick] coordinates {
(1,16.25170045905277)
(2,16.495877702855157)
(3,9.737392576668832)
(4,6.711517597633478)
(5,5.423892639065195)
(6,4.453238891131238)
	};	
\addplot[color=magenta,mark=otimes,mark size=4pt,ultra thick] coordinates {
(1,1.481463553979728)
(2,1.232773495398006)
(3,1.125118770263264)
(4,1.016110730044176)
(5,0.844438484649703)
(6,0.6512687621406819)
	};	
			\addplot[color=green,mark=diamond,mark size=4pt,ultra thick] coordinates {
(1,1.7994571724208919)
(2,1.7410183112795672)
(3,2.286846094762936)
(4,1.3511768980358858)
(5,1.282397223295495)
(6,1.1617025857688235)

	};
			\addplot[color=cyan,mark=+,mark size=4pt,ultra thick] coordinates {
(1,4.4784886424764534)
(2,4.8597400198979477)
(3,4.369106284961381)
(4,4.560998587487884)
(5,4.764325415885782)
(6,5.756795515340624)
	};	
\legend{Kmeans,Bayes,SVM,lr,lda,pca}
  

           \nextgroupplot[
        legend pos=north east,
        legend cell align=left,
%		title=the impact of Memory on Executor Size,
		xlabel=Executor size,
		ylabel=GC time/Total time (\%),
		label style={font=\Huge},
		title style={font=\Huge},
		legend style={font=\Large},
		ymax=40,
		ytick={0,10,...,40},
		xtick={1,2,...,6},
		xticklabels={size1,size2,size3,size4,size5,size6},
		]

		\addplot[color=blue,mark=o,mark size=4pt,ultra thick] coordinates {
(1,1.4711718651407697)
(2,1.9466654555296543)
(3,2.518262086972089)
(4,2.4183340441776453)
(5,2.1210497928052634)
(6,1.5732079530812297)


	};	
	%file {
%evaluation/evaluation_kmeans3d.dat
%};
		\addplot[color=purple,mark=x, mark size=4pt,ultra thick] coordinates {
(1,8.086576190808154)
(2,6.547572651170337)
(3,3.7807990669003773)
(4,2.848321597212583)
(5,2.4860971142364976)
(6,1.2974573614427505)

	};		
	
	\addplot[color=black,mark=triangle,mark size=4pt,ultra thick] coordinates {
    
(1,3.8108889612685553)
(2,3.76102661843985)
(3,2.421489538869425)
(4,1.8767414544348242)
(5,1.7989274591355389)
(6,1.3011337589062781)
	};		

\legend{Join,Aggregate, Scan}

\end{groupplot}    
\end{tikzpicture}




